Toward Metrics for Differentiating Out-of-Distribution Sets

Vanilla CNNs, as uncalibrated classifiers, suffer from classifying out-of-distribution (OOD) samples nearly as confidently as in-distribution samples. To tackle this challenge, some recent works have demonstrated the gains of leveraging available OOD sets for training end-to-end calibrated CNNs. However, a critical question remains unanswered in these works: how to differentiate OOD sets for selecting the most effective one(s) that induce training such CNNs with high detection rates on unseen OOD sets? To address this pivotal question, we provide a criterion based on generalization errors of Augmented-CNN, a vanilla CNN with an added extra class employed for rejection, on in-distribution and unseen OOD sets. However, selecting the most effective OOD set by directly optimizing this criterion incurs a huge computational cost. Instead, we propose three novel computationally-efficient metrics for differentiating between OOD sets according to their "protection" level of in-distribution sub-manifolds. We empirically verify that the most protective OOD sets -- selected according to our metrics -- lead to A-CNNs with significantly lower generalization errors than the A-CNNs trained on the least protective ones. We also empirically show the effectiveness of a protective OOD set for training well-generalized confidence-calibrated vanilla CNNs. These results confirm that 1) all OOD sets are not equally effective for training well-performing end-to-end models (i.e., A-CNNs and calibrated CNNs) for OOD detection tasks and 2) the protection level of OOD sets is a viable factor for recognizing the most effective one. Finally, across the image classification tasks, we exhibit A-CNN trained on the most protective OOD set can also detect black-box FGS adversarial examples as their distance (measured by our metrics) is becoming larger from the protected sub-manifolds.

==> some_comparison.tex <==


\begin{comment}

\begin{table}
    \centering
    \resizebox{0.5\textwidth}{!}{
\begin{tabular}{cccc}
&& \multicolumn{2}{c}{Unseen OOD sets}\\
\cline{3-4}
In-distribution& Seen OOD set & Avg AUROC ($\uparrow$)& Avg FPR @95\%TPR ($\uparrow$) \\
\hline
\multirow{2}{*}{ SVHN } & $\ddagger$ISUN & \underline{94.73} & \underline{31.97} \\
& LSUN & 99.25 & 4.39 \\
& C10 & 99.75 & 0.41 \\
& $\star$C100 & \textbf{99.86} & \textbf{0.08} \\
& T-ImgNt & 99.75 & 1.10 \\
\hline

\multirow{2}{*}{ CIFAR-10 } & $\ddagger$SVHN & \underline{86.38} & \underline{75.04} \\
& T-ImgNt & \textbf{93.89} & 34.44\\
&LSUN & 93.31	&	38.59	\\
& $\star$C100* & 93.03	&	\textbf{26.13}\\ 
\end{tabular} }
\caption{Performance of calibrated vanilla CNN trained on each seen OOD set and tested on all unseen OOD sets to report average of AUROC and FPR.}
\label{calib-CNN}
 
\end{table}


%mahalonobis tuned by only one OOD set
\begin{table*}
    \centering
    \begin{tabular}{cccc}
In-distribution & Seen OOD set& Calibrated CNN  & Mahalonobis-detector  \\
&& AUROC/FPR &  AUROC/FPR\\
\hline
\multirow{5}{*}{ svhn }& $\ddagger$ISUN & 94.73/31.97& 98.89/4.7 \\
& LSUN & 99.25/ 4.39 & 98.91/4.43 \\
& C10 & 99.75/0.41 & 99.03/3.82 \\

& T-ImgNt & 99.75/1.10 & 98.89/ 4.46 \\
& $\star$C100 & \textbf{99.86/0.07} & \textbf{99.09/ 3.53} \\
\hline
\multirow{5}{*}{ cifar10 } &  $\ddagger$SVHN & 86.38 /75.04 & 90.29/ 35.78 \\

& ISUN & 86.20/77.03& 91.26/ 35.62 \\
& LSUN & 93.31/ 38.59 & 91.27/ 36.37 \\
&T-ImgNt & \textbf{93.89}/34.44 & 91.86/ 33.02 \\
&$\star$C100* & 93.03/\textbf{26.13} & \textbf{93.59/ 29.96} \\

\hline

\end{tabular} 
    \caption{Caption}
    \label{tab:my_label}
\end{table*}





\begin{table}
    \centering
    \resizebox{0.5\textwidth}{!}{
\begin{tabular}{cccc}
&& \multicolumn{2}{c}{Unseen OOD sets}\\
\cline{3-4}
In-distribution& Seen OOD set & Avg AUROC ($\uparrow$)& Avg FPR @95\%TPR ($\uparrow$) \\
\hline
\multirow{2}{*}{ SVHN } & $\ddagger$ISUN & \underline{94.73} & \underline{31.97} \\
& LSUN & 99.25 & 4.39 \\
& C10 & 99.75 & 0.41 \\
& $\star$C100 & \textbf{99.86} & \textbf{0.08} \\
& T-ImgNt & 99.75 & 1.10 \\
\hline

\multirow{2}{*}{ CIFAR-10 } & $\ddagger$SVHN & \underline{86.38} & \underline{75.04} \\
& T-ImgNt & \textbf{93.89} & 34.44\\
&LSUN & 93.31	&	38.59	\\
& $\star$C100* & 93.03	&	\textbf{26.13}\\ 
\end{tabular} }
\caption{Performance of calibrated vanilla CNN trained on each seen OOD set and tested on all unseen OOD sets to report average of AUROC and FPR.}
\label{calib-CNN}
 
\end{table}


%mahalonobis tuned by only one OOD set
\begin{table*}
    \centering
    \begin{tabular}{cccc}
In-distribution & Seen OOD set& Calibrated CNN  & Mahalonobis-detector  \\
&& AUROC/FPR &  AUROC/FPR\\
\hline
\multirow{5}{*}{ svhn }& $\ddagger$ISUN & 94.73/31.97& 98.89/4.7 \\
& LSUN & 99.25/ 4.39 & 98.91/4.43 \\
& C10 & 99.75/0.41 & 99.03/3.82 \\

& T-ImgNt & 99.75/1.10 & 98.89/ 4.46 \\
& $\star$C100 & \textbf{99.86/0.07} & \textbf{99.09/ 3.53} \\
\hline
\multirow{5}{*}{ cifar10 } &  $\ddagger$SVHN & 86.38 /75.04 & 90.29/ 35.78 \\

& ISUN & 86.20/77.03& 91.26/ 35.62 \\
& LSUN & 93.31/ 38.59 & 91.27/ 36.37 \\
&T-ImgNt & \textbf{93.89}/34.44 & 91.86/ 33.02 \\
&$\star$C100* & 93.03/\textbf{26.13} & \textbf{93.59/ 29.96} \\

\hline

\end{tabular} 
    \caption{Caption}
    \label{tab:my_label}
\end{table*}

\end{comment}
\begin{comment}

\subsection{Comparison with Related Works}

\begin{table*}[h]
 \centering
 \small
 \resizebox{0.7\textwidth}{!}{
\begin{tabular}{ccc}
In-dist. Task & Methods &In-dis Rej. (FNR)$\downarrow$ $/$  Avg OOD Rej. (TNR)$\uparrow$\\
    
\hline
 \multirow{3}{*}{SVHN} & Baseline& $4.06$ / $58.07$\\
 		
 &ODIN & $4.71$ / $69.34$\\
&Mahalanobis Detector& $6.40$ / $97.41$ \\
&A-VGG$^{\star}$& $\textbf{0.34}$ / $\textbf{99.88}$\\
\hline


\multirow{3}{*}{CIFAR-10} & Baseline& $7.01$ / $44.81$\\
&ODIN & $5.81$ / $65.74$\\
&Mahalanobis Detector& $5.90$ / $80.68$\\
&A-VGG$^{\star}$ & $\textbf{5.65}$ / $\textbf{85.10}$ \\
\hline
\multirow{3}{*}{Urban-Sound}& Baseline& $22.83$ / $40.96$\\
&  ODIN & $27.38$ / $47.45$\\
&Mahalanobis Detector& $16.13$ / $45.42$\\
&A-CNN$^{\star}$& $\textbf{12.02}$ / $\textbf{55.40}$\\
\end{tabular} }
     \caption{Comparison of A-CNN$^{\star}$ with state-of-the-art approaches according to average rejection rates (TNR) of OOD sets and in-distribution rejection rate (FNR). Details are given in the supplementary.}
     \label{related-works}
     
 \end{table*}
We compare A-CNN$^{\star}$ with three state-of-the-art methods, including baseline~\cite{hendrycks2016baseline}, ODIN~\cite{liang2017principled}, and Mahalanobis-distance-based detector~\cite{lee2018simple} (briefly called Mahalanobis detector)\footnote{\scriptsize{We use publicly-available Github codes of the state-of-the-art OOD detectors.}}. These approaches attempt to detect OOD samples according to a specific threshold on the modified calibrated predictive confidence scores. As mentioned earlier, TNR and FNR of these methods are the same concept as OOD rejection rate and in-distribution rejection rate, respectively. 

To set all hyper-parameters of these baselines, including threshold, we use two validation sets with $1000$ samples each, for in-distribution and each OOD set. For ODIN, we find the optimal magnitude noise from $\{0.0, 0.0005, 0.0014, 0.001, 0.01 \}$ and temperature set to $1000$ for all experiments. For Mahalanobis-detector, the optimal magnitude of noise is selected among $\{0.0, 0.005, 0.002, 0.0014, 0.001, 0.0005\}$. To set a threshold for each OOD set, we set it such as to achieve $95\%$ TPR on the validation set. Then, using the optimal tuned hyper-parameters (including threshold), we perform OOD detection process on test OOD sets and test in-distribution set, reporting TNR and FNR, respectively. 


Note these approaches (mahalanobis detector and ODIN) originally reported TPR (= 1-FNR), FPR (= 1-TNR), and detection rate~\cite{lee2018simple,liang2017principled} by setting the best threshold for each test set. However, more fair setting would be finding the optimal threshold using a separate validation set (for each test set), then applying it for the test set. However, we believe setting a separate threshold for each OOD set even by using a distinct validation set is still unrealistic since in real-world scenarios, it is unknown the coming samples belong to which OOD set for setting its proper threshold. Therefor, the major challenge for the threshold-based approach is setting a global threshold, which shall leads to a global high detection rate on all OOD sets.



Therefore, a comparison of the performances of the threshold-based approaches (which thresholds are fixed using validation sets) and A-CNN (as non-threshold-based approach) presents in Table~\ref{related-works}. As it can be seen, A-CNN$^{\star}$ performs \emph{significantly} better than these threshold-based approaches when comparing average OOD rejection and in-distribution rejection rates.

 \end{comment}  









